PAL: Persona-Augmented Emotional Support Conversation Generation

Due to the lack of human resources for mental health support, there is an increasing demand for employing conversational agents for support. Recent work has demonstrated the effectiveness of dialogue models in providing emotional support. As previous studies have demonstrated that seekers' persona is an important factor for effective support, we investigate whether there are benefits to modeling such information in dialogue models for support. In this paper, our empirical analysis verifies that persona has an important impact on emotional support. Therefore, we propose a framework for dynamically inferring and modeling seekers' persona. We first train a model for inferring the seeker's persona from the conversation history. Accordingly, we propose PAL, a model that leverages persona information and, in conjunction with our strategy-based controllable generation method, provides personalized emotional support. Automatic and manual evaluations demonstrate that PAL achieves state-of-the-art results, outperforming the baselines on the studied benchmark. Our code and data are publicly available at https://github.com/chengjl19/PAL.

==> sections/acknowledgement.tex <==
This work was supported by the National Science Foundation for Distinguished Young Scholars
(with No. 62125604) and the NSFC projects (Key
project with No. 61936010 and regular project with
No. 61876096). This work was also supported
by the Guoqiang Institute of Tsinghua University,
with Grant No. 2019GQG1 and 2020GQG0005,
and sponsored by Tsinghua-Toyota Joint Research
Fund.


==> sections/persona_extractor.tex <==
As mentioned above, it is important to study persona information in the emotional support task. Anticipating a seeker's persona information in advance is often impossible, so it is necessary to infer possible persona information from what the seeker has said.

\subsection{Problem Definition and Implementation} \label{bart model}
Assuming that a dialogue between two people, A and B, can be represented as $ U=\{u_1^A, u_1^B, u_2^A, u_2^B,..., u_n^A, u_n^B\} $ and each agent has a set of persona information $ P_A = \{p_1^A, ..., p_{mA}^A\} $ and $ P_B = \{p_1^B, ..., p_{mB}^B\} $. Specifically, we use the dataset Persona-chat \cite{zhang2018personalizing}, where each piece of data consists of a conversation between two people and their respective persona information. Our task is to use what a person has said to predict his or her persona information. For example, using agent A's said sentences $ U_A = \{u_1^A, u_2^A,..., u_n^A\} $ to predict $ P_A $. We fine-tune bart-large-cnn with lr 1e-5 to accomplish this task.

\subsection{Individualized Emotional Support Conversation}
Using the fine-tuned model described in \S\ref{bart model}, we can provide the ESConv \cite{liu2021towards} dataset with the inferred persona information annotations for each round of conversation. Since the beginning rounds of this dataset are generally in greeting, we provide the annotations starting from the third round of conversation, an example of which is shown in the table \ref{persona annotation example}. We refer to this dataset with additional annotations later as IESConv.

\begin{table*}[]
\begin{tabular}
	{
    >{
    \centering\arraybackslash}p{
    0.2\textwidth}
	>{
    \arraybackslash}p{
    0.7\textwidth}}
\toprule
\multirow{3}{*}{Conversation} 
& Seeker:    hello \\
& Supporter: Hi there! How may I support you today? \\  
& Seeker:    I'm just feeling anxious about my job future. A lot of my colleagues are having trouble getting their licenses because of covid which means we wont be able to work. \\
\midrule
Persona information & i am worried about my job future.\\
\midrule
\multirow{2}{*}{Conversation} 
& Supporter: That must be hard. COVID has really turned our world upside down! What type of occupation are you in \\  
& Seeker:    I'm studying to be a pharmacist. \\
\midrule
\multirow{2}{*}{Persona information} 
& i am worried about my job future. \\ 
& I'm studying to be a pharmacist \\
\bottomrule
\end{tabular}
\caption{IESConv data example. There are 5 utterances in this example dialogue. The persona information annotation in IESConv starts from the third utterance, after that each time seeker says a sentence there will be persona information annotation inferred from all the previous words spoken by seeker.}
\label{persona annotation example}
\end{table*}

\subsection{Relevance of Individualization and Seeker Evaluation}
To verify that modeling persona information in the emotional support task is indeed important, we perform an analysis using our IESConv. 
As described by \citeauthor{liu2021towards}, the ESConv is scored by workers at the following aspects: (1) the supporter's empathy level, (2) the relevance of the topic and the supporter's responses, (3) the seeker's emotional intensity. We analyze these three metrics separately and use the average cosine similarity of responses and persona information in a conversation to represent how closely the responses and persona information are combined. To transform the sentences into vectors, we used two methods: SimCSE \cite{gao2021simcse}, a sentence embedding model trained with a contrast learning approach, and fasttext \cite{joulin2017bag}, using which we can present a sentence with averaged word embeddings. The results using SimCSE are shown in figure \ref{fig:simcse analysis}, and the results using fasttext can be found in appendix \ref{appendix: analysis}.
It can be seen that the conversations with higher empathy, relevance, or emotion intensity decrease (this can be seen as emotion improvement) scores have higher similarity to persona information. This further illustrates the necessity of modeling persona information in the emotional support task.

\begin{figure*}[h]
\centering
\subfigure[Result of empathy]{
\begin{minipage}[t]{0.3\linewidth}
\centering
\includegraphics[width=2in, height=1.5in]{fig/simcse_empathy.png}
\end{minipage}
}
\subfigure[Result of relevance]{
\begin{minipage}[t]{0.3\linewidth}
\centering
\includegraphics[width=2in, height=1.5in]{fig/simcse_relevance.png}
\end{minipage}
}
\subfigure[Result of emotion intensity decrease]{
\begin{minipage}[t]{0.3\linewidth}
\centering
\includegraphics[width=2in, height=1.5in]{fig/simcse_emotion_intensity_decrease.png}
\end{minipage}
}
\centering
\caption{The relationship between empathy score, relevance score, emotion intensity decrease score, and similarity of responses to persona information using SimCSE. In general, the higher the score, the higher the similarity.}
\label{fig:simcse analysis}
\end{figure*}
